Efficient and DoS-resistant Consensus for Permissioned Blockchains

Existing permissioned blockchain systems designate a fixed and explicit group of committee nodes to run a consensus protocol that confirms the same sequence of blocks among all nodes. Unfortunately, when such a permissioned blockchain runs in a large scale on the Internet, these explicit committee nodes can be easily turned down by denial-of-service (DoS) or network partition attacks. Although work proposes scalable BFT protocols that run on a larger number of committee nodes, their efficiency drops dramatically when only a small number of nodes are attacked. In this paper, our EGES protocol leverages Intel SGX to develop a new abstraction called "stealth committee", which effectively hides the committee nodes into a large pool of fake committee nodes. EGES selects a distinct group of stealth committee for each block and confirms the same sequence of blocks among all nodes with overwhelming probability. Evaluation on typical geo-distributed settings shows that: (1)EGES is the first permissioned blockchain's consensus protocol that can tolerate tough DoS and network partition attacks; and (2) EGES achieves comparable throughput and latency as existing permissioned blockchains' protocols

==> 8related.tex <==
% \section{Related Work}\label{sec:related}

% \textbf{Public Blockchains.}
% % % \textit{Proof of Work.} 
% Public blockchains mainly reside in two categories: PoW and PoS. PoW was first
% proposed by BitCoin~\cite{nakamoto2008bitcoin} and myriad of subsequent works
% improve multiple aspects of it, including performance
% ), sharding
% ( ), and
% . Among them, ByzCoin is most related to
% \xxx as it use PoW to select committee nodes and runs a byzantine agreement on
% these nodes. However, ByzCoin relies on structural communication and explicit
% membership, making it vulnerable to targeted DoS attacks.  

% PoS systems (\algorand~\cite{gilad2017algorand, micali2016algorand},
% , ) select consensus
% nodes with the probability proportional to each nodes' wealth (\ie, stake) in
% the system. All these systems but algorand leverages variants of the
% longest-chain rule to confirm blocks and thus are vulnerable to partition
% attacks. \xxx is compared to Algorand both qualitatively 
% (\chref{sec:background:public}) and quantitively (\chref{sec:eval:perf}).
% Overall, \xxx is complementary to Algorand: Algorand is more suitable for a
% public cryptocurrency, while \xxx is robust and efficient in a large-scale
% permissioned blockchain. 

% One key
% differences between \xxx and public blockchains is that public blockchains uses
% the real-world market value of cryptocurrency to encourage users to follow the
% protocol, while \xxx targets on non-cryptocurrency semantics and leverages SGX
% to enforce users to follow the protocol~\chref{motivation}.

% Public blockchains rely on cryptocurrencies, and \xxx aims 
% to be orthogonal to currencies. 

% The ration is that the more stake a node holds, the more incentive
% it has to maintain the well being of the system. One major drawback of public
% blockchain systems is that they rely on the value of the cryptocurrency to
% abstract users and encourage them to follow the protocol. 

% {When the market
% value of the cryptocurrency oscalite. the safety of the system cannot be
% ensured.}






% is the first PoW
% based blockchain system that works as a fully functional cryptocurrency system,
% but it suffers from huge energy consumption and bad performance.
% Bitcoin-NG~\cite{eyal2016bitcoinng} and Fruitchain~\cite{pass2016fruitchains}
% use multiple types of blocks to improve the throughput of Bitcoin.
% GHOST~\cite{sompolinsky2013accelerating} proposes to select a subtree rather
% than the longest chain when the blockchain forks to reduce wasted blocks.
% Ethereum~\cite{buterin2014ethereum, wood2014ethereum} reduces the difficulty of
% hash computations in PoW and introduces the uncle block mechanism to reduce
% potential forks. Solidus~\cite{abraham2016solidus},
% ByzCoin~\cite{kokoris2016enhancing}, PeerCensus~\cite{decker2016bitcoin}, and
% Hybrid Consensus~\cite{pass2016hybrid} use PoW to select a group of committee
% and runs a byzantine fault tolerant (BFT) protocols~\cite{pbft:osdi99} to
% achieve consensus on a single block. 
% Elastico~\cite{luu2016secure} and OmniLedger~\cite{kokoris2017omniledger}
% propose a sharding approach inspired by traditional database to linearly scale 
% existing blockchains' throughput. 
% These works improves the throughput and
% latency of PoW based blockchain but still consume large amount of energy.
% Moreover, the BFT protocols assume more than two thirds of the selected
% committee members are honest. \xxx{} has good performance and does not assume
% the honesty of the nodes. 



% {
% It assumes an extremely powerful adversary that can compromise the
% committee members once they send out packets, so it lets each committee member to
% determine whether it is a committee member independently, and proposes a
% customized byzantine agreement protocol to let each committee only sends one
% messages in each round. \xxx{} differs from \algorand in three aspects. First,
% to preserve strong consistency, \algorand assumes a vast majority (\eg{} 80\%)
% of the users to be honest because it works on arbitrarily devices, while \xxx{}
% does not need this assumption by leveraging SGX. As shown in our evaluation
% (\S\ref{sec:eval:robust}), \xxx{} proceeds correctly even when more than 20\% of nodes
% are offline. Second, \algorand strongly tolerates DoS attacks because each node
% only sends out one message in each round; \xxx{} uses non-acceptors to generate
% fake votes to cover the real stealth acceptors (\chref{partition}), so \xxx{} 
% tolerates DoS attack for these acceptors (slightly weaker than \algorand).
% Third, \xxx{}'s protocol has few parameters (Table~\ref{tab:parameters}), and
% \algorand has 12 parameters.
% }

% are two PoS systems similar to \algorand that
% each node independently determines whether it is the proposer of next block.
% Praos uses a secure multi-party computation algorithm; Snow-white uses a
% PoW similar hash computation mechanism and set each node's hash target according
% to their stakes. is a PoS system that uses off-band methods
% (\ie{} selling tokens) to elect 49 super nodes and runs a BFT protocol in a 21
% node committee with this 49 super nodes to append new blocks. Unlike \xxx, PoS
% systems often require a vast majority of nodes to be honest. 

% \textit{Others.} 
% SpaceMint~\cite{park2018spacemint} elects the proposer based on 
%  their storage space dedicated for the system. 
 
%  SlimCoin~\cite{slimcoin}
%  proposes the idea of proof of burn, where a node must destroy some amount of its coins 
%  to become the next proposer. 

\bfheading{Permissioned Blockchains and BFT protocols.} 
Multiple Works improve the efficiency and scalability of BFT protocols for
permissioned blockchains. SBFT~\cite{SBFT}, CoSi~\cite{syta2016keeping}, and
FastBFT~\cite{liu2016scalable} use threshold signatures~\cite{cachin2005random,
shoup2000practical} to reduce the message complexity of PBFT to linear;
Zyzzyva~\cite{zyzzyva:sosp07}, WHEAT~\cite{sousa2015separating} uses speculative
execution to improve the throughput of PBFT; HoneyBadger~\cite{miller2016honey}
and BEAT~\cite{duan2018beat} are two practical BFT protocols to achieve liveness
on asynchronous network; A2M~\cite{chun2007attested},
TrInc~\cite{levin2009trinc}, CheapBFT~\cite{kapitza2012cheapbft},
MinBFT~\cite{veronese2013efficient}, and Hybster~\cite{bft:eurosys17} use
trusted hardwares to restricts the behavior of malicious nodes in BFT. These
works are orthogonal to \xxx because all of them run on a set of fixed consensus
nodes, while \xxx handles DoS attacks on committee nodes. 

Stellar~\cite{mazieres2015stellar} and Ripple~\cite{schwartz2014ripple} divide
the network into small groups called federates. Consensus is achieved first in
each federate and then among federates. Prior works~\cite{gilad2017algorand,
kim2017enhancing, dinh2017untangling} point out, this federate approach requires
manually assigning trust relations among nodes. Unlike \xxx, existing
permissioned blockchains are efficient for small scale applications, but are not
designed for large scale deployment on the Internet.

% but are not designed to work in the
% Internet scale. 

\bfheading{SGX and Blockchain Applications}. 
% Diverse applications have been developed on
% blockchains. 
% Ethereum and introduces EVM, a
% deterministic runtime, to run smart contract applications on all consensus nodes
% of a blockchain. 
Hawk~\cite{kosba2016hawk} and zkLedger~\cite{narula17zkledger} focus on
enhancing confidentiality of smart contracts~\cite{buterin2014ethereum}.

%  works similar as Ekiden.
%   To deploy an
% application in Ekiden or ShadowEth, these application has to be mostly
% re-written using the smart contract language~\cite{buterin2014ethereum}. 
% Ekiden and ShadowEth are applications on top of blockchains.
BlockStack~\cite{ali2016blockstack} builds a decentralized DNS and storage
services on blockchains. 
% and only a small portion of an application's state (\eg{}
% checkpoints) is appended to \xxx blockchain.
TeeChain~\cite{teechain} is a payment network and leverages SGX to prevent
parties from misbehaving. Overall, \xxx's consensus protocol is complementary to
these application systems and can be integrated in their underlying consensus
layer.
%TODO
% \textbf{BFT protocols}.Cosi, pbft, scalable bft.


% Multiple byzantine fault tolerant protocols~\cite{crain2017leader,
% ren2017practical, abraham2017efficient,micali2017byzantine,
% beerliova2007efficient, alchieri2008byzantine, kapron2008fast,
% okun2008efficient, clement2009making, singh2009zeno, correia2010asynchronous,
% delporte2011byzantine, groce2012byzantine, veronese2013efficient,
% mostefaoui2014signature, luu2015scp} are proposed for private blockchains.
% HLF~\cite{sousa2017byzantine} is a high performance  byzantine fault tolerant
% ordering service for Hyperledger. Stellar~\cite{stellar} introduces a new
% consensus module where each node has different quoroums. 


\textbf{SGX-powered Blockchains.} SGX improves diverse aspects of blockchain
systems.  
% Proof of
% Luckpresents a protocol that lets each miner seal a
% random number generated from SGX into the block as the ``luck'' of the block.
% The protocol selects the chain with the largest accumulative luck as the winner.
% This protocol will have inconsistency (forks) when the network is temporarily
% partitioned because the partitions will confirm different largest accumulative
% % luck. 
% CoCo~\cite{azure:coco} is an ongoing permissioned blockchain project that
% can support diverse consensus protocol (\eg{} Raft~\cite{raft:usenix14}) in
% SGX-powered nodes. CoCo does not include a consensus protocol.

% \.
% \scifer{} uses SGX's attestation feature to defend against sybil attacks, and
% runs an ``ages''-based voting algorithm to select a block proposer. However, the
% consensus algorithm is run outside of SGX, so the safety of this protocol has to
% assume a vast majority of nodes to be honest. 


% ; \xxx's safety does not rely on any
% node's honesty.
% {Algorand solves the targeting attack by let each node only send out one packet
% in each round. However, this approach is not efficient because it needs all
% messages to be P2P broadcasts and need up to 13 rounds to complete. Compared
% with Algorand, the stealth acceptor not only simplifies the protocol, but also
% improves the the efficiency.
% }


% [TODO] Discussion on Hybster
% [TODO] disucss about conflict txns. 
% [TODO] Discussion on the safety of SGX. It can protect against false positive. 
